Towards Semantically Enriched Embeddings for Knowledge Graph Completion

Embedding based Knowledge Graph (KG) Completion has gained much attention over the past few years. Most of the current algorithms consider a KG as a multidirectional labeled graph and lack the ability to capture the semantics underlying the schematic information. In a separate development, a vast amount of information has been captured within the Large Language Models (LLMs) which has revolutionized the field of Artificial Intelligence. KGs could benefit from these LLMs and vice versa. This vision paper discusses the existing algorithms for KG completion based on the variations for generating KG embeddings. It starts with discussing various KG completion algorithms such as transductive and inductive link prediction and entity type prediction algorithms. It then moves on to the algorithms utilizing type information within the KGs, LLMs, and finally to algorithms capturing the semantics represented in different description logic axioms. We conclude the paper with a critical reflection on the current state of work in the community and give recommendations for future directions.

==> tex/related_work.tex <==
%\section{Related Work}\label{sec:related-work}

Several recent studies have been published discussing the existing approaches for KG completion or refinement  In~\cite{Paulheim17}, the authors provide a survey of the articles related to KG refinement including various classical and rule-based approaches methods for KG completion. This study is more general as compared to the existing surveys which are specifically focused on KG embedding based methods. One such survey organizes the algorithms for KG completion using KG embeddings based on scoring functions such as translational models, semantic matching models, etc.~\cite{WangMWG17}. However, this survey does not discuss the methodologies proposed for kg completion using multimodal information given in KGs such as images, text, and numeric literals. In~\cite{DBLP:journals/semweb/GeseseBAS21}, categorize these methods based on scoring function inspired by~\cite{WangMWG17} as well as based on each of the modalities. The survey shows theoretical and experimental comparisons of the existing approaches. In~\cite{BianchiRCPM20}, the authors briefly introduce KG embedding methods and provide insight into the explainability aspects of these methods. As compared to these existing studies, this article targets the semantic aspects of these methods by summarizing and discussing the approaches that have been proposed so far for leveraging semantics provided in the KG.
%\ma{to be added to intro ... paragraph ... or subsection...}

==> tex/table_evaluation_protocol.tex <==
\begin{table}[t] 
\centering
\caption{Overview of the tasks and the datasets used for evaluation for each of the categories.}
\begin{tabular}{p{3.5cm}|p{5.5cm}|p{5.25cm} } 
\toprule
\textbf{Category}& \textbf{Tasks}&  \textbf{Datasets}\\ \midrule

Transductive Link Prediction& Link Prediction, Triple Classification, Entity Classification  & FB15K\textcolor{blue}{~\cite{bordes2011learning}}, FB15K-237\textcolor{blue}{~\cite{toutanova-chen-2015-observed}}, WN18\textcolor{blue}{~\cite{bordes2011learning}}, WN18RR\textcolor{blue}{~\cite{dettmers2018convolutional}}, YAGO3-10\textcolor{blue}{~\cite{dettmers2018convolutional}}, LiterallyWikidata\textcolor{blue}{~\cite{GeseseAS21}} \\ \hline

Inductive Link Prediction &Link Prediction, Triple Classification &Wikidata5M\textcolor{blue}{~\cite{Wang2021KEPLERAU}}, Wikidata68K\textcolor{blue}{~\cite{GeseseSA22}, ILPC 2022~\cite{abs-2203-01520}} \\ \hline

LLM-Based Methods & Link Prediction & FB15K237, WN18RR, FB15K-237N, FB15K-237NH, Wiki27K~\textcolor{blue}{\cite{LvL00LLLZ22}}, OpenBG500, Nell-One\textcolor{blue}{~\cite{XiongYCGW18}}  \\ \hline
%mehwish: FB15K-237N, FB15K-237NH, Wiki27K~\cite{LvL00LLLZ22} all of these are introduced in this paper
Methods using Type-Hierarchy& Link Prediction, Entity Type Prediction& WN18RR, WN18, FB15k, FB15KET, YAGO43KET\textcolor{blue}{~\cite{10.1145/3132847.3133095}}, FB15K+\textcolor{blue}{~\cite{xie2016representation}}, FB15K*, JF17K\textcolor{blue}{~\cite{ZhangKWM18}}, NELL-995\textcolor{blue}{~\cite{WangWHLG21}},  YAGO26K-906, DB111K-174\textcolor{blue}{~\cite{Xie2016DKRL}}.\\ \hline
%mehwish: NELL-995 find ref.
Methods using Description Logic Axioms& Inductive Reasoning (Subsumption, Class Membership), Deductive Reasoning (Unsatisfiability of the named concept, predicting axioms in deductive closure of an ontology)  & FoodOn\textcolor{blue}{~\cite{Dooley2018FoodOnAH}}, HeLIS\textcolor{blue}{~\cite{DragoniBME18}}, GO\textcolor{blue}{~\cite{KulmanovH17}}, SNOMED-CT\textcolor{blue}{~\cite{Donnelly2006SNOMEDCTTA}}, GALEN\textcolor{blue}{~\cite{Pole1996TheGH}}, Anatomy\textcolor{blue}{~\cite{Mungall2012UberonAI}}, PPI\textcolor{blue}{~\cite{SzklarczykMC0WS17}}, FOBI, NRO\textcolor{blue}{~\cite{abs-2305-07163}} \\ 

%\textbf{Feature}&\textbf{Twitter}&\textbf{TREC}&\textbf{MR}&\textbf{AG News}\\
%\textbf{Sampling Method}&\textbf{Accuracy}\\
%\hline\hline
%Random  & 0.887 \\

%\hline
%nearest-neighbor & 0.71

%\\
%\hline
%CPC subclass &0.70
%\\
\bottomrule
\end{tabular}
\label{table:evaluation_protocol}
\end{table}

==> tex/table_logic_old.tex <==
\begin{table}[t!]
    \centering
    \caption{Axioms in $\mathcal{EL}^{++}$, $\mathcal{ALC}$, and $\mathcal{SH}$}
    \label{tab:logic}
    \begin{tabular}{lll}
        \toprule
         $\mathcal{EL}^{++}$ & $\mathcal{ALC}$ & $\mathcal{SH}$ \\
         \midrule
         Top ($\top$), Bottom ($\bot$) & Top ($\top$), Bottom ($\bot$) & Top ($\top$), Bottom ($\bot$) \\
         Nominal Constructor & Nominal Constructor & Nominal Constructor \\
         (Binary) Role Assertion & (Binary) Role Assertion & (Binary) Role Assertion \\
         Concept Assertion & Concept Assertion & Concept Assertion \\
         Concept Intersection ($\sqcap$) & Concept Intersection ($\sqcap$) & Concept Intersection ($\sqcap$) \\
         Concept Subsumption ($\sqsubseteq$) & Concept Subsumption ($\sqsubseteq$) & Concept Subsumption ($\sqsubseteq$) \\
         -- & Concept Union ($\sqcup$) & Concept Union ($\sqcup$) \\
         -- & Concept Negation ($\neg$) & Concept Negation ($\neg$) \\
         Existential Quantification ($\exists$) &  Existential Quantification ($\exists$) & Existential Quantification ($\exists$) \\ 
        -- & Universal Quantification ($\forall$) &  Universal Quantification ($\forall$) \\
        -- & -- & Role Subsumption ($\sqsubseteq$) \\
        -- & -- & Role Transitivity \\ 
        
        \bottomrule
    \end{tabular}
\end{table}

==> tex/table_overview.tex <==
% Please add the following required packages to your document preamble:

\begin{table}[t!]
\caption{Comparison of the expressivity of semantically enriched embeddings. Notation: $a,b$ are instances, $C,D,E$ are concepts, $r, r_1, r_2, s$ are relations. The symbol \cmark (resp. (\cmark) indicates that it has been demonstrated by construction or empirically that the approach supports (resp. partially) the expression; otherwise, \xmark is indicated. }
\label{tab:semantic_embeddings}
\footnotesize
\begin{tabular}{llcccccccc}
\hline
                                & Expressions                     & ELEm           & EMEL++         & BoxEL        & ELBE           & Box$^2$EL    & CatE           & OWL2Vec*    & TransOWL \\ \hline
\multirow{5}{*}{Constructors}                 & $\bot$                          & \cmark   & \cmark   & \cmark & \cmark   & \xmark     & \xmark       & \xmark    & \xmark\\
                                     & $\top$                          & \xmark       & \xmark       & \xmark     & \xmark       & \xmark     & \cmark   & \cmark & \xmark\\
                                     & $\{a\}$                           & (\cmark) & \xmark       & \cmark & \xmark       & \cmark & \xmark       & \xmark    & \cmark \\
                                     & $C(a)$                          & \cmark   & \cmark   & \cmark & \cmark   & \cmark & \xmark       & \cmark  & \cmark \\
                                     & $r(a,b)$                        & \cmark   & \cmark   & \cmark & \cmark   & \cmark & \xmark       & \cmark  & \cmark \\ \hline
\multirow{7}{*}{$\mathcal{EL}^{++}$} & $C \sqsubseteq D$               & \cmark   & \cmark   & \cmark & \cmark   & \cmark & \cmark   & \cmark  & \cmark \\
                                     & $C \sqcap D \sqsubseteq E$      & (\cmark) & \cmark   & \cmark & \cmark   & \cmark & (\cmark) & \xmark    & \xmark \\
                                     & $\exists r.C \sqsubseteq D$     & \cmark   & \cmark   & \cmark & \cmark   & \cmark & \cmark   & \cmark & \cmark \\
                                     & $C  \sqsubseteq \exists r.D$    & \cmark   & \cmark   & \cmark & \cmark   & \cmark & \cmark   & \cmark & \cmark \\
                                     & $C \sqcap D \sqsubseteq \bot$   & \xmark       & \cmark   & \cmark & \cmark   & \cmark & \cmark   & \xmark   &  \xmark  \\
                                     & $\exists r.C \sqsubseteq \bot $ & (\cmark) & (\cmark) & \cmark & (\cmark) & \cmark & \xmark       & \xmark   &  \xmark  \\
                                     & $ C  \sqsubseteq \bot $         & \xmark       & \cmark   & \cmark & \cmark   & \cmark & \xmark       & \xmark    & \xmark \\ \hline
\multirow{5}{*}{$\mathcal{ALC}$}     & $C \sqcup D$                    & \xmark       & \xmark       & \xmark     & \xmark       & \xmark     & \cmark   & \xmark     & \xmark \\
                                     & $\forall r.D$                   & \xmark       & \xmark       & \xmark     & \xmark       & \xmark     & \cmark   & \xmark   &  \xmark \\
                                     & $\neg C$                        & \xmark       & \xmark       & \xmark     & \xmark       & \xmark     & \cmark   & \xmark   &  \xmark \\
                                     & $C \sqsubseteq \forall r.D$     & \xmark       & \xmark       & \xmark     & \xmark       & \xmark     & \xmark       & \cmark & \cmark\\
                                     & $\forall r.C \sqsubseteq D$     & \xmark       & \xmark       & \xmark     & \xmark       & \xmark     & \xmark       & \cmark & \cmark \\
\midrule
\multirow{2}{*}{$\mathcal{SH}$}      & $r \sqsubseteq s$               & \xmark       & \cmark   & \xmark     & \xmark       & \xmark     & \xmark       & \cmark & \cmark \\
                                     & $r_1 \circ r_2 \sqsubseteq s$   & \xmark       & \cmark   & \xmark     & \xmark       & \xmark     & \xmark       & \cmark & \xmark \\ 
\bottomrule
\end{tabular}
\end{table}
